Experimentally Tractable Generation of High-Order Rogue Waves in Bose-Einstein Condensates

In this work, we study a prototypical, experimentally accessible scenario that enables the systematic generation of so-called high-order rogue waves in atomic Bose-Einstein condensates. These waveforms lead to significantly and controllably more extreme focusing events than the famous Peregrine soliton. In one spatial dimension, we showcase conclusive numerical evidence that our scheme generates the focusing behavior associated with the first four rogue waves from the relevant hierarchy. We then extend considerations to anisotropic two-dimensional and even three-dimensional settings, establishing that the scheme can generate second order rogue waves despite the well-known limitation of finite-time blow up of focusing nonlinear Schr\"odinger equations.

==> header.tex <==
\usepackage{tabularx,amsmath,amsfonts,boxedminipage,graphicx,mathtools,appendix,physics}
\usepackage{tabularx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{boxedminipage}
\usepackage{appendix}
\usepackage{algorithm2e}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{subfigure}
\usepackage{cite}
%\usepackage[margin=1in,letterpaper]{geometry} % this shaves off default margins which are too big
%\numberwithin{equation}{section}
%\numberwithin{figure}{section}
\RestyleAlgo{boxruled}
\usepackage[utf8]{inputenc}

\usepackage[font=small]{caption}
\usepackage[labelformat=empty, position=top]{subcaption}
\usepackage{graphicx}
\usepackage[export]{adjustbox}

\usepackage{csquotes}
\MakeOuterQuote{"}


\usepackage{hyperref} % adds hyper links inside the generated pdf file
 \hypersetup{%
 	colorlinks=true,       % false: boxed links; true: colored links
 	linkcolor=blue,          % color of internal links
 	citecolor=blue,        % color of links to bibliography
 	filecolor=magenta,      % color of file links
 	urlcolor=blue         
 }
%%%
\usepackage{floatrow}
\usepackage{lmodern}

\newcommand{\Tee}{\mathsf{T}}
%\graphicspath{{figures/}}

% \setlength{\abovecaptionskip}{-1pt}
% \addtolength{\subfigcapskip}{-10pt}

\newcommand{\includegraphicsTwoDown}[2]{
  \begin{subfigure}[t]{0.05\textwidth}
    \textbf{(a)}
  \end{subfigure}
  \begin{subfigure}[t]{0.93\textwidth}
    \includegraphics[width=\linewidth, valign=t]{#1}
  \end{subfigure}\hfill \\ \vspace{3mm}
  \begin{subfigure}[t]{0.05\textwidth}
    \textbf{(b)}
  \end{subfigure}
  \begin{subfigure}[t]{0.93\textwidth}
    \includegraphics[width=\linewidth, valign=t]{#2}
  \end{subfigure}
}

\newcommand{\includegraphicsTwoAcross}[2]{
  \begin{subfigure}[t]{0.05\textwidth}
    \textbf{(a)}
  \end{subfigure}
  \begin{subfigure}[t]{0.43\textwidth}
    \includegraphics[width=\linewidth, valign=t]{#1}
  \end{subfigure}
  \begin{subfigure}[t]{0.05\textwidth}
    \textbf{(b)}
  \end{subfigure}
  \begin{subfigure}[t]{0.43\textwidth}
    \includegraphics[width=\linewidth, valign=t]{#2}
  \end{subfigure}
}

\newcommand{\includegraphicsTwoByTwo}[4]{
  \begin{subfigure}[t]{0.05\textwidth}
    \textbf{(a)}
  \end{subfigure}
  \begin{subfigure}[t]{0.03\textwidth}
    \includegraphics[width=\linewidth, valign=t]{#1}
  \end{subfigure}
  \begin{subfigure}[t]{0.05\textwidth}
    \textbf{(b)}
  \end{subfigure}
  \begin{subfigure}[t]{0.03\textwidth}
    \includegraphics[width=\linewidth, valign=t]{#2}
    \hfill \\ \vspace{3mm}
    \end{subfigure}
  \begin{subfigure}[t]{0.05\textwidth}
    \textbf{(c)}
  \end{subfigure}
  \begin{subfigure}[t]{0.03\textwidth}
    \includegraphics[width=\linewidth, valign=t]{#3}
  \end{subfigure}
  \begin{subfigure}[t]{0.05\textwidth}
    \textbf{(d)}
  \end{subfigure}
  \begin{subfigure}[t]{0.03\textwidth}
    \includegraphics[width=\linewidth, valign=t]{#4}    
  \end{subfigure}
}

\newcommand{\includegraphicsFourAcross}[4]{
  \begin{subfigure}[t]{0.025\textwidth}
    \textbf{(a)}
  \end{subfigure}
  \begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=\linewidth, valign=t]{#1}
  \end{subfigure}
  \begin{subfigure}[t]{0.025\textwidth}
    \textbf{(b)}
  \end{subfigure}
  \begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=\linewidth, valign=t]{#2}
  \end{subfigure}  
  \begin{subfigure}[t]{0.025\textwidth}
    \textbf{(c)}
  \end{subfigure}
  \begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=\linewidth, valign=t]{#3}
  \end{subfigure}
  \begin{subfigure}[t]{0.025\textwidth}
    \textbf{(d)}
  \end{subfigure}
  \begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=\linewidth, valign=t]{#4}   
  \end{subfigure} 
}
